What to look at and where: Semantic and Spatial Refined Transformer for detecting human-object interactions

We propose a novel one-stage Transformer-based semantic and spatial refined transformer (SSRT) to solve the Human-Object Interaction detection task, which requires to localize humans and objects, and predicts their interactions. Differently from previous Transformer-based HOI approaches, which mostly focus at improving the design of the decoder outputs for the final detection, SSRT introduces two new modules to help select the most relevant object-action pairs within an image and refine the queries' representation using rich semantic and spatial features. These enhancements lead to state-of-the-art results on the two most popular HOI benchmarks: V-COCO and HICO-DET.

==> content/tables.tex <==
\begin{table*}[]
%\hskip1.0cm
\begin{adjustbox}{width=\columnwidth*2,center}
\centering
\begin{tabular}{|l|l|c|c|c|c|c|c|}
\hline
Method                                & Feature Backbone & Full(def) & Rare(def) & None-Rare(def) & Full(ko) & Rare(ko) & None-Rare(ko) \\ \hline
UnionDet~\cite{kim2020detecting}      & ResNet50-FPN     & 17.58     & 11.72     & 19.33          & 19.76    & 14.68    & 21.27         \\
IPNet~\cite{wang2020learning}         & Hourglass-104    & 19.56     & 12.79     & 21.58          & 22.05    & 15.77    & 23.92         \\
PPDM~\cite{liao2020ppdm}              & Hourglass-104    & 21.1      & 14.46     & 23.09          & -        & -        & -             \\
Functional~\cite{bansal2020detecting} & ResNet-101       & 21.96     & 16.43     & 23.62          & -        & -        & -             \\
Hou et al.~\cite{hou2020visual}       & ResNet-50        & 23.63     & 17.21     & 25.55          & 25.98    & 19.12    & 28.03         \\
ConsNet~\cite{liu2020consnet}         & ResNet-50        & 24.39     & 17.1      & 26.56          & -        & -        & -             \\
DRG~\cite{gao2020drg}                 & ResNet50-FPN     & 24.53     & 19.47     & 26.04          & 27.98    & 23.11    & 29.43         \\
IDN~\cite{IDN}                        & ResNet-50        & 26.29     & \textbf{22.61}     & 27.39          & 28.24    & \textbf{24.47}    & 29.37         \\ \hline
GTNet                                 & ResNet-50        & 26.78     & 21.02     & 28.5           & 28.80     & 22.19    & 30.77         \\
GTNet                                 & ResNet-152       & \textbf{28.30}      & 22.02     & \textbf{30.16}          & \textbf{30.31}    & 23.63    & \textbf{32.30}          \\ \hline \hline
iCAN~\cite{gao2018ican}                                  & ResNet-50        & 33.38     & 21.43     & 36.95          & -        & -        & -             \\
Li et al.~\cite{li2019transferable}                       & ResNet-50        & 34.26     & 22.9      & 37.65          & -        & -        & -             \\
Peyre et al.~\cite{peyre2019detecting}                               & ResNet-50-FPN    & 34.35     & 27.57     & 36.38          & -        & -        & -             \\
IDN~\cite{IDN}                                   & ResNet-50        & 43.98     & \textbf{40.27}     & 45.09          & -        & -        & -             \\ \hline
GTNet                                 & ResNet-50        & 44.71     & 33.8      & 47.97          & 44.71    & 33.8     & 47.97         \\
GTNet                                 & ResNet-152       & \textbf{46.78}     & 34.87     & \textbf{50.34}          & \textbf{46.78}    & \textbf{34.87}    & \textbf{50.34}         \\ \hline
\end{tabular}
\end{adjustbox}
\vspace{0.08cm}
\caption{\small \it Performance comparisons in the HICO-DET~\cite{chao2018learning} test set. . }
\label{tab:hico-det_t}
\vspace{-0.4cm}
\end{table*}

%  In full setting all test images are used for evaluation. In rare and non-rare setting two smaller separate sets of test images are used for evaluation. These sets are created on the basis of the number of training samples
\begin{table}[]
%\hskip1.0cm
\begin{adjustbox}{width=\columnwidth,center}
\centering
\begin{tabular}{|l|l|c|c|}
\hline
Method                                   & Feature Backbone & Scenario 1    & Scenario 2    \\ \hline
T. Wang et. al.~\cite{wang2019deep}      & ResNet-50        & 47.3          & -             \\
DRG~\cite{gao2020drg}                    & ResNet50-FPN     & 51.0          & -             \\
VSGNet~\cite{ulutan2020vsgnet}           & ResNet - 152     & 51.8          & 57.0          \\
Wan et al.~\cite{wan2019pose}            & ResNet50-FPN     & 52.0          & -             \\
Zhong et al.~\cite{zhong2020polysemy}    & ResNet - 152     & 52.6          & -             \\
H. Wang et.al.~\cite{wang2020contextual} & ResNet50-FPN     & 52.7          & -             \\
Kim et al.~\cite{kim2020detecting}       & ResNet - 152     & 53.0          & -             \\
Liu et al.~\cite{liuamplifying}          & ResNet-50        & 53.1          & -             \\
ConsNet~\cite{liu2020consnet}                       & ResNet-50        & 53.2          & -             \\
IDN~\cite{IDN}                           & ResNet-50        & 53.3          & 60.3          \\
OSGNet~\cite{zhang2020improved}                           & ResNet-152        & 53.4          &    -      \\
Sun et al.~\cite{sun2020human}           & ResNet - 101     & 55.2          & -             \\
DIRV~\cite{fang2020dirv}                 & EfficientDet-d3  & 56.1          & -             \\ \hline
GTNet                                    & ResNet-50        & 56.2          & 60.1          \\
\textbf{GTNet}                           & ResNet-152       & \textbf{58.3} & \textbf{61.9} \\ \hline
\end{tabular}
\end{adjustbox}
\vspace{0.08cm}
\caption{\small \it Performance comparisons in the  V-COCO~\cite{gupta2015visual} test set. Many current works do not report their models' performance in Scenario 2.}
\label{tab:v-coco}
\vspace{-0.4cm}
\end{table}

\begin{table*}[]
%\hskip1.0cm
\begin{adjustbox}{width=\columnwidth*2,center}
\centering
\begin{tabular}{|l|l|c|c|c|c|c|c|}
\hline
Method                                & Feature Backbone       & Full(def) & Rare(def) & None-Rare(def) & Full(ko) & Rare(ko) & None-Rare(ko) \\ \hline
VSGNet                                & ResNet-152             & 19.8      & 16.05     & 20.91          & -        & -        & -             \\
FCMNet                                & ResNet-50              & 20.41     & 17.34     & 21.56          & 22.04    & 18.97    & 23.12         \\
ACP                                   & ResNet-152             & 20.59     & 15.92     & 21.98          & -        & -        & -             \\
PD-Net                                & ResNet-152             & 20.81     & 15.9      & 22.28          & 24.78    & 18.88    & 26.54         \\
DJ-RN                                 & Resnet-50 and PointNet & 21.34     & 18.53     & 22.18          & 23.69    & 20.64    & 24.6          \\
OSGNet                                & ResNet-152             & 21.4      & 18.12     & 22.38          & -        & -        & -             \\
DIRV                                  & EfficientDet-d3        & 21.78     & 16.38     & 23.39          & 25.52    & 20.84    & 26.92         \\
ConsNet                               & ResNet-50              & 22.15     & 17.12     & \textbf{23.65}          & -        & -        & -             \\
IDN                                   & ResNet-50              & \textbf{23.36}     & \textbf{22.47}     & 23.63          & \textbf{26.43}    & \textbf{25.01}    & \textbf{26.85}         \\ \hline 
GTNet                                 & ResNet-50              & 20.87     & 17.51     & 21.88          & 23.72    & 19.56    & 24.97         \\ 
GTNet                                 & ResNet-152             & 22.28     & 17.87     & 23.6           & 25.24    & 20.66    & 26.61         \\ \hline \hline

\end{tabular}
\end{adjustbox}
\vspace{0.08cm}
\caption{\small \it Performance comparisons in the HICO-DET~\cite{chao2018learning} test set.  }
\label{tab:hico-det_f}
\vspace{-0.4cm}
\end{table*}
%  In full setting all test images are used for evaluation. In rare and non-rare setting two smaller separate sets of test images are used for evaluation. These sets are created on the basis of the number of training samples.





\begin{table}[]
%\hskip0.3cm
%\begin{adjustbox}{width=\columnwidth}
\centering
\begin{tabular}{|c|c|c|}
\hline
Number of  Channels & \multicolumn{1}{l|}{Scenario 1} & \multicolumn{1}{l|}{Scenario 2} \\ \hline
64                  & 57.21                           & 61.1                            \\
128                 & 57.46                           & 61.6                            \\
256                 & 57.48                           & 61.25                           \\
512                 & 58.29                           & 61.85                           \\ \hline
\end{tabular}
%\end{adjustbox}
\vspace{0.1cm}
\caption{\small \it Performance of GTNet with different number of channels for key and value.}
\label{tab:oracle}
\vspace{-0.4cm}
\end{table}

